Differentiable Scaffolding Tree for Molecular Optimization

The structural design of functional molecules, also called molecular optimization, is an essential chemical science and engineering task with important applications, such as drug discovery. Deep generative models and combinatorial optimization methods achieve initial success but still struggle with directly modeling discrete chemical structures and often heavily rely on brute-force enumeration. The challenge comes from the discrete and non-differentiable nature of molecule structures. To address this, we propose differentiable scaffolding tree (DST) that utilizes a learned knowledge network to convert discrete chemical structures to locally differentiable ones. DST enables a gradient-based optimization on a chemical graph structure by back-propagating the derivatives from the target properties through a graph neural network (GNN). Our empirical studies show the gradient-based molecular optimizations are both effective and sample efficient. Furthermore, the learned graph parameters can also provide an explanation that helps domain experts understand the model output.

==> DST arxiv/additional_experiment.tex <==




\section{Baseline Setup}
\label{sec:baseline}

In this section, we describe the experimental setting for baseline methods. 
Most of the settings follow the original papers. 
\begin{itemize}
\item \textbf{LigGPT} (string-based distribution learning model with Transformer as a decoder)~\cite{bagal2021liggpt} is trained for 10 epochs using the Adam optimizer with a learning rate of $6e-4$. 
LigGPT comprises stacked decoder blocks, each of which, is composed of a masked self-attention layer and fully connected neural network. 
Each self-attention layer returns a vector of size 256, that is taken as input by the fully connected network. The hidden layer of the neural network outputs a vector of size 1024 and uses a GELU activation and the final layer again returns a vector of size 256 to be 7 used as input for the next decoder block. LigGPT consists of 8 such decoder blocks. LigGPT has around 6M parameters. 
\item \textbf{GCPN} (Graph Convolutional Policy Network)~\cite{You2018-xh} leveraged graph convolutional network and policy gradient to optimize the reward function that incorporates target molecular properties and adversarial loss. 
In each step, the allowable action to the current molecule could be either connecting a new substructure or an atom with an existing molecular graph or adding a bond to connect existing
atoms. GCPN predicts the actions and is trained via proximal policy optimization (PPO) to optimize an accumulative reward, including molecular property objectives and adversarial loss. 
Both policy network and adversarial network (discriminative training) use the same neural architecture, which is a three-layer graph convolutional network (GCN)~\cite{kipf2016semi} with 64 hidden nodes. Batch normalization is adopted after each layer, and sum-pooling is used as the aggregation function. Adam optimizer is used with 1e-3 initial learning rate, and batch size is 32.  



\item \textbf{MolDQN} (Molecule Deep Q-Networks)~\cite{zhou2019optimization}, same as GCPN, formulate the molecule generation procedure as a Markov Decision Process (MDP) and use Deep Q-Network to solve it. 
The reward includes target property and similarity constraint. 
Following the original paper, the episode number is 5,000, maximal step in each episode is 40. Each step calls oracle once; thus, 200K oracle calls are needed in one generation process. 
The discount factor is 0.9. 
Deep Q-network is a multilayer perceptron (MLP) whose hidden dimensions are 1024, 512, 128, 32, respectively. The input of the Q-network is the concatenation of the molecule feature (2048-bit Morgan fingerprint, with a radius of 3) and the number of left steps. 
Adam is used as an optimizer with 1e-4 as the initial learning rate.
Only rings with a size of 5 and 6 are allowed. 
It leverages $\epsilon$-greedy together with randomized value functions (bootstrapped-DQN) as an exploration policy, $\epsilon$ is annealed from 1 to 0.01 in a piecewise linear way. 
\item \textbf{GA+D} (Genetic Algorithm with Discriminator network)~\cite{nigam2019augmenting} uses a deep neural network as a discriminator to enhance exploration in a genetic algorithm. 
$\beta$ is an important hyperparameter that weights the importance of the discriminator's loss in the overall fitness function, and we set it to 10. 
The generator runs 100 generations with a population size of 100 for \textit{de novo} molecular optimization and 50 generations with a population size of 50 for molecular modification. 
Following the original paper~\cite{nigam2019augmenting}, the architecture of the discriminator is a two-layer fully connected neural network with ReLU activation and a sigmoid output layer. The hidden size is 100, while the size of the output layer is 1. 
The input feature is a vector of chemical and geometrical properties characterizing the molecules. 
We used Adam optimizer with 1e-3 as the initial learning rate. 
\item \textbf{RationaleRL}~\cite{jin2020multi} is a deep generative model that grows a molecule atom-by-atom from an initial rationale (subgraph). 
The architecture of the generator is a message-passing network (MPN) followed by MLPs applied in breadth-first order. The generator is pre-trained on general molecules combined with an encoder and then fine-tuned to maximize the reward function using policy gradient. 
The encoder and decoder MPNs both have hidden dimensions of 400. The dimension of the latent variable is 20. Adam optimizer is used on both pre-training and fine-tuning with initial learning rates of 1e-3, 5e-4, respectively. The annealing rate is 0.9. We pre-trained the model with 20 epochs. 

% These rationales are identified from molecules as substructures that are likely responsible for each property of interest. We then learn to expand rationales into a full molecule using graph generative models. Our final generative model composes molecules as mixtures of multiple rationale completions, and this mixture is fine-tuned to preserve the properties of interest. 

\item \textbf{MARS}~\cite{xie2021mars} leverage Markov chain Monte Carlo sampling (MCMC) on molecules with an annealing scheme and an adaptive proposal. The proposal is parameterized by a graph neural network, which is trained on MCMC samples. 
We follow most of the settings in the original paper. 
The message passing network has six layers, where the node embedding size is set to 64. 
Adam is used as an optimizer with 3e-4 initial learning rate. To generate a basic unit, top-1000 frequent fragments are drawn from ZINC database~\cite{sterling2015zinc} by enumerating single bonds to break.  
During the annealing process, the temperature $T = 0.95^{\lfloor t/5\rfloor}$ would gradually decrease to 0. 
% % \item \textbf{MIMOSA}~\cite{fu2021mimosa} also reformulate molecule optimization as a sampling problem and the property oracles are encoded in the target distribution. We use Adam optimizer with a learning rate of 0.001. For pretraining, we follow~\cite{hu2019strategies} to set GNNs with 5 layers and 300-d hidden units. 
% For mGNN, we randomly mask a single node for each molecule, while for bGNN, we randomly select a leaf node for each molecule. When training them, we choose batch size 256, epochs number 10, and learning rate $1e^{-3}$. Then, during inference stage, we keep 20 molecules each iteration. 
% Burn-in is intended to give the Markov Chain time to reach its equilibrium distribution, particularly if it has started from a lousy starting point.  We select $T_{\text{burnin}}$ from $\{1,3,5,10\}$ and find $T_{\text{burnin}}=5$ works best in most of the setting. If $T_{\text{burnin}}$ is too small, the Markov chain would mix slowly. In addition, we set $T_{\text{max}} = 10$. 
\end{itemize}



\section{Implementation Details}
\label{sec:implementation_details}

\subsection{Dataset}
\label{sec:dataset}
We use ZINC 250K dataset, which contains around 250K druglike molecules extracted from the ZINC
database~\cite{sterling2015zinc}. 
The clean data is available at \cite{huang2021therapeutics,du2021graphgt} (\url{https://tdcommons.ai/generation_tasks/molgen/}). 
We first clean the data by removing the molecules containing out-of-vocabulary substructure and having 195K molecules left.
% We randomly select 80\% data as training set and 10\% data as validation set. 
% For goal-directed molecule optimization, the selection criteria for test set is (1) QED score is less than 0.6; (2) JNK3 and GSK3\bm{$\beta$} scores are less than 0.02; (3) LogP score is less than -1. From the selected molecules, we randomly select 500 molecules as test set. De novo molecule generation do not require test set. 

\textbf{Vocabulary $\calS$: set of substructure}. 
The substructure is the basic building block in our method, including frequent atoms and rings. 
On the other hand, atom-wise molecule generation is difficult due to the existence of rings. 
To select the substructure set $\calS$, we break all the ZINC molecules into substructures (including single rings and single atoms), count their frequencies, and include the substructures whose frequencies are higher than 1000 into vocabulary set $\calS$. 
The final vocabulary contains 82 substructures, including the frequent atoms like carbon atom, oxygen atom, nitrogen atom, and frequent rings like benzene ring. 
The vocabulary size is big enough for this proof-of-concept study. 
Other works also need to constrain their design space, such as MolDQN only allowing three types of atoms in a generation: ``C'', ``N'', ``O''~\cite{zhou2019optimization};  JTVAE~\cite{jin2018junction,jin2019learning}, as well as RationaleRL~\cite{jin2020multi} only using frequent substructures similar to our setting. 
On the other hand, we may not want infrequent atoms or substructures because rare substructures in ZINC may have some undesired properties such as toxicity, may not be stable, may not be easily synthesizable~\cite{gao2020synthesizability}. 
Also, rare substructures may impede the learning of oracle GNN. 
Note that users can enlarge the substructure space when they apply our method. 
We show all the 82 substructures in $\calS$ in Figure~\ref{fig:vocab}. 



% The vocabulary size is, of course, a limitation, but we think it is enough for proof-of-concept work at this moment. Other works also need to constrain their design space, such as MolDQN only allowing three types of atoms in a generation: C, N, O; JTVAE, as well as RationaleRL only using frequent substructures similar to our setting. On the other hand, we may not want infrequent atoms or substructures because rare substructures in ZINC may have some undesired properties such as toxicity, may not be stable, may not be easily synthesizable. 



\subsection{Software/Hardware Configuration}
\label{sec:hardware_config}
We implemented \mname using Pytorch 1.7.0, Python 3.7, RDKit v2020.09.1.0 on an Intel Xeon E5-2690 machine with 256G RAM and 8 NVIDIA Pascal Titan X GPUs. 




\subsection{Target molecular properties}
\label{sec:property}
{Target molecular properties} include
\begin{itemize}
\item \textbf{QED} represents a quantitative estimate of drug-likeness. QED score ranges from 0 to 1. It can be evaluated by the RDKit package (\url{https://www.rdkit.org/}). 
\item \textbf{LogP} represents octanol-water partition coefficient, measuring molecules' solubility. LogP score ranges from $-\infty$ to $+\infty$. Thus, when optimizing LogP individually, we use the GNN model to do regression. 
\item \textbf{SA} (Synthetic Accessibility) score measures how hard it is to synthesize a given molecule, based on a combination of the molecule’s fragments contributions~\cite{ertl2009estimation}. 
It is evaluated via RDKit~\cite{landrum2006rdkit}. 
The raw SA score ranges from 1 to 10. A higher SA score means the molecule is hard to be synthesized and is not desirable. 
In the multiple-objective optimization, we normalize the SA score to $[0,1]$ so that a higher normalized SA value mean easy to synthesize. 
Following~\cite{gao2020synthesizability}, we use the normalize function for raw SA score, 
\begin{equation*}
\text{normalized-SA}(X)=
\left\{
\begin{array}{ll}
1,  & \text{SA}(X) < \mu \\
\exp{(-\frac{(\text{SA}(X) - \mu)^2}{2\sigma^2})},  &  \text{SA}(X) \geq \mu, \\
\end{array}
\right. 
\end{equation*}
where $\mu = 2.230044, \sigma = 0.6526308$. 
\item \textbf{JNK3} (c-Jun N-terminal Kinases-3) belongs to the mitogen-activated protein kinase family and are responsive to stress stimuli, such as cytokines, ultraviolet irradiation, heat shock, and osmotic shock. Similar to GSK3\bm{$\beta$}, JNK3 is also evaluated by well-trained\footnote{The test AUROC score is 0.86~\cite{jin2020multi}. } random forest classifiers using ECFP6 fingerprints using ExCAPE-DB dataset~\cite{li2018multi,jin2020multi}, and the range is also $[0,1]$. 
\item \textbf{GSK3\bm{$\beta$}} (Glycogen synthase kinase 3 beta) is an enzyme that in humans is encoded by the GSK3\bm{$\beta$} gene. Abnormal regulation and expression of GSK3\bm{$\beta$} is associated with an increased susceptibility towards bipolar disorder. It is evaluated by well-trained\footnote{The test AUROC score is also 0.86~\cite{jin2020multi}. }  random forest classifiers using ECFP6 fingerprints using ExCAPE-DB dataset~\cite{li2018multi,jin2020multi}. GSK3\bm{$\beta$} score of a molecule ranges from 0 to 1. 
\end{itemize}
For QED, LogP, normalized SA, JNK3, and {GSK3\bm{$\beta$}}, higher scores are more desirable under our experimental setting. 



\subsection{Evaluation metrics}
\label{sec:metrics}
We leverage the following {evaluation metrics} to measure the optimization performance:  
\begin{itemize}
\item \textbf{Novelty} is the fraction of the generated molecules that do not appear in the training set. 
\item  \textbf{Diversity} of generated molecules is defined as the average pairwise Tanimoto distance between the Morgan fingerprints~\cite{You2018-xh,jin2020multi,xie2021mars}. 
\begin{equation}
\text{diversity} = 1 - \frac{1}{|\calZ|(|\calZ|-1)}\sum_{Z_1,Z_2 \in \calZ} \text{sim}(Z_1,Z_2),
\end{equation}
where $\calZ$ is the set of generated molecules. $\text{sim}(Z_1,Z_2)$ is the Tanimoto similarity between molecule $Z_1$ and $Z_2$. 
\item \textbf{(Tanimoto) Similarity} measures the similarity between the input molecule and generated molecules. 
It is defined as
\[
\text{sim}(X,Y) = \frac{\bfb_{X}^\top \bfb_{Y}}{\Vert \bfb_{X}\Vert_2 \Vert \bfb_{Y}\Vert_2}, 
\] 
$\bfb_{X}$ is the binary Morgan fingerprint vector for the molecule $X$. In this paper, it is a 2048-bit binary vector. 
\item \textbf{SR} (Success Rate) is the percentage of the generated molecules that satisfy the property constraint measured by objective $f$ defined in Equation~\eqref{eqn:objective}.  
For single-objective \textit{de novo} molecular generation, the objective $f$ is the property score, the constraints for JNK3, GSK3\bm{$\beta$} and LogP are JNK3$\geq 0.5$, GSK3\bm{$\beta$}$\geq 0.5$ and LogP$\geq5.0$ respectively. 
For multi-objective \textit{de novo} molecular generation, the objective $f$ is the average of all the normalized target property scores. Concretely, when optimizing ``JNK3+GSK3\bm{$\beta$}'', both JNK3 and GSK3\bm{$\beta$} ranges from 0 to 1, $f$ is average of JNK3 and GSK3\bm{$\beta$} scores; when optimizing ``{QED+SA+JNK3+GSK3\bm{$\beta$}}'', we first normalized SA to 0 to 1. $f$ is average of QED, normalized SA, JNK3 and GSK3\bm{$\beta$} scores. 
The constraint is the $f$ score is greater than 0.4. 
\item \textbf{\# of oracle calls} during the generation process. \mname needs to call oracle in labeling data for GNN and \mname based \textit{de novo} generation, thus we show the costs for both steps. 
\item \textbf{chemical validities}. 
As we only enumerate valid chemical structures during the recovery from scaffolding trees (Section~\ref{sec:assemble}), the chemical validities of the molecules produced by \mname are always 100\%. 
% \item \textbf{Objective $f$ Value} (Eqn~\ref{eqn:f}). 
% \item \textbf{Molecular Properties} are the main target of optimization and would be evaluated. Detailed description of these properties are in Section~\ref{sec:property}. 
\end{itemize}
% Novelty and diversity are the metrics on the set of generated molecules, are evaluated only in de novo generation task. In contrast, similarity and SR focus on single molecule and are only evaluated in goal-oriented optimization task. 


\begin{figure}[h!]
\centering
\includegraphics[width=12.8cm]{figure/vocabulary.png}
\caption{All the substructures in the vocabulary set $\calS$, drawn from ZINC 250K database~\cite{sterling2015zinc}. It includes atoms and single rings appearing more than 1000 times in the ZINC250K database. 
}
\label{fig:vocab}
\end{figure}


\subsection{Assembling Molecule from Scaffolding Tree}
\label{sec:assemble}

Each scaffolding tree corresponds to multiple molecules due to rings' multiple combination ways. For each scaffolding tree, we enumerate all the possible molecules following~\cite{jin2018junction} for further selection. We provide two examples in Figure~\ref{fig:assemble} to illustrate it. Two examples are related to ring-atom combination and ring-ring combination, respectively. For ring-ring combination, our current setting does not support the spiro compounds (contains rings sharing one atom but no bonds) or phenalene-like compounds (contains three rings sharing one atom, and each two of them sharing a bond). These two cases are relatively rare chemical structures in the context of drug discovery~\cite{supsana2005thermal}. 
As we only enumerate valid chemical structures during the recovery from scaffolding trees, the chemical validities are always 100\%.
% Though these two cases are relatively rare chemical structures, the limiting chemical space is a potential limitation of our current model.

\begin{figure}[h!]
\centering
\subfigure[Ring-atom connection. When connecting atom and ring in a molecule, an atom can be connected to any possible atoms in the ring. In the example, there are 4 possible ways to add a Chlorine atom (``Cl'') as an expansion node to the target ring, which is a leaf node in the scaffolding tree. ]{
\includegraphics[width=12cm]{figure/assemble1.png}}
\subfigure[Ring-ring connection. When connecting ring and ring, there are two general ways, (1) one is to use a bond (single, double, or triple) to connect the atoms in the two rings. (2) another is two rings share two atoms and one bond. 
In the example, there are 14 possible ways to add a Cyclohexane ring (SMILES is ``C1CCCCC1'') and connect it to the target ring, which is a leaf node in the scaffolding tree. ]{
\includegraphics[width=12.9cm]{figure/assemble2.png}}
\caption{Assemble examples. 
}
\label{fig:assemble}
\end{figure}

\subsection{Details on GNN Learning and \mname Optimization}
\label{sec:gnn_setup}

Both the size of substructure embedding and hidden size of GCN (GNN) in Eq.~\eqref{eqn:gcn} are $d=100$. 
The depth of GNN $L$ is 3.  
When training GNN, the training epoch number is 5, and we evaluate the loss function on the validation set every 20K data passes. 
When the validation loss would not decrease, we terminate the training process. 
During the inference procedure, we set the maximal iteration to 5k. 
When optimizing ``JNK3'', ``GSK3\bm{$\beta$}'', ``QED'', ``JNK3+GSK3\bm{$\beta$}'' and ``QED+SA+JNK3+GSK3\bm{$\beta$}'', we use binary cross entropy as loss criterion. 
When optimizing ``LogP'', since LogP ranges from $-\infty$ to $+\infty$, we leverage GNN to conduct regression tasks and use mean square error (MSE) as loss criteria $\calL$. 
In \textit{the de novo} generation, in each generation, we keep $C=10$ molecules for the next iteration. 
In most cases in experiment, the size of the neighborhood set (Definition.~\ref{def:neighbor}) is less than 100. 
We use Adam optimizer with 1e-3 learning rate in training and inference procedure, optimizing the GNN and differentiable scaffolding tree, respectively. 
When optimizing \mname, our method processes one \mname at a time. As a complete generation algorithm, we optimize a batch parallelly and select candidates based on DPP. 
we set the iteration $T$ to a large enough number and tracked the result. When editing cannot improve the objective function or use up oracle budgets, we stop it. All results in the tables are from experiments up to $T=50$ iterations. 




\subsection{Results of Different Random Seeds}
\label{sec:error_bar}
In this section, we present the empirical results that use different random seeds for multiple runs. 
In our pipeline, the random error comes from in two steps: 
(1) Training oracle GNN: data selection/split, training process including data shuffle and GNN's parameter initialization. 
(2) Inference (Optimizing \mname): before optimizing \mname, we initialize the learnable parameter randomly, including $\widetilde{\bfN}$, $\widetilde{\bfw}$, $\widetilde{\bfA}$, which also brings randomness.  
To measure the robustness of the proposed method, we use 5 different random seeds for the whole pipeline and compare the difference of 5 independent trials. 
The results are reported in Table~\ref{table:errorbar}. We find that almost all the metrics would not changes significantly among various trials, validating the robustness of the proposed method. 

\begin{table*}[h!]
\tiny
\centering
\caption{Results of 5 independent trials using different random seeds. For novelty, diversity and SR (success rate), we report the average value of 5 runs and their standard deviation.  }
\label{table:errorbar}
 \resizebox{0.6\textwidth}{!}{
\begin{tabular}{ccccc}
\toprule[0.6pt]
Tasks & Novelty$\uparrow$ & Diversity$\uparrow$ & SR$\uparrow$ & \# Oracles$\downarrow$ \\
\hline 
JNK3 & 98.1\%$\pm$0.3\% & 0.722$\pm$0.032 &  92.8\%$\pm$0.5\% & 10K+5K\\ 
GSK3\bm{$\beta$}& 98.6\%$\pm$0.5\% & 0.738$\pm$0.047 & 91.8\%$\pm$0.3\% & 10K+5K\\ 
LogP &  100.0\%$\pm$0.0\% & 0.716$\pm$0.032 &  100.0\%$\pm$0.0\% & 10K+5K\\ 
JNK3+GSK3\bm{$\beta$} & 98.6\%$\pm$1.1\% & 0.721$\pm$0.021 & 91.3\%$\pm$0.6\% & 10K+5K\\ 
QED+SA+JNK3+GSK3\bm{$\beta$} &  99.2\%$\pm$0.3\% & 0.731$\pm$0.029 & 79.4\%$\pm$1.2\% & 20K+5K\\ 
\bottomrule[0.6pt]
\end{tabular}}
\end{table*}


\subsection{Complexity Analysis}
\label{sec:complexity} 

We did computational analysis in terms of oracle calls and computational complexity. 
(1) \textbf{oracle calls}. DST requires $O(TM)$ oracle calls, where $T$ is the number of iterations (Alg~\ref{alg:main}). 
$M$ is the number of generated molecules (Equation.~\ref{eqn:dpp_obj}), we have $M\leq K_{\text{}}J$, $K_{\text{}}$ is the number of nodes in the scaffolding tree, for small molecule, $K_{\text{}}$ is very small. 
$J$ is the number of enumerated candidates in each node. As shown in Figure~\ref{fig:assemble}, $J$ is also upper-bounded ($J\leq 4+14$ for the example in Figure~\ref{fig:assemble}). 
(2) \textbf{computational complexity}. 
The computational complexity is $O(TMC^2)$ (the main bottleneck is DPP method, Algorithm~\ref{alg:dpp_greedy}), where the size of selected molecules $C=10$ for all the tasks (Section~\ref{sec:dpp} \&~\ref{sec:gnn_setup}). 
For all the tasks in Table~\ref{table:denovo_single} and~\ref{table:denovo_multi}, DST can be finished in 12 hours on an Intel Xeon E5-2690 562 machine with 256G RAM and 8 NVIDIA Pascal Titan X GPUs. 
The complexity and runtime are acceptable for molecule optimization. 




\section{Additional Experimental Results}
\label{sec:additional_experiment}
In this section, we present the additional empirical results, including additional results on \textit{de novo} generation, ablation study, chemical space visualization, interpretability analysis (case study). 



\iffalse
\subsection{Learning Curve of \mname on \textit{de novo} Molecule Generation}
\label{sec:learn_curve}
We show the change of average objective as a function of generations in Figure~\ref{fig:learning_curve}. 
The objective includes $f$-value, GNN prediction (i.e., $\hat{y}$ in Equation~\eqref{eqn:gnn}) and target properties. 
We find (1) the $f$'s value, JNK3 and GSK3\bm{$\beta$} grow steadily while QED and LogP maintain a high value, indicating that our method is able to generate molecules with desirable properties; (2) the real objective $f$'s value and the GNN's prediction $\haty$ show the similar value, thus validating the GNN is well-trained and can be used as a differentiable proxy as the black-box oracle. 

\begin{figure}[h!]
\centering
\subfigure[f vs GNN]{
\includegraphics[width=5cm]{figure/fscore_t1.png}}
\subfigure[Property]{
\includegraphics[width=5cm]{figure/fscore_t2.png}}
\caption{Learning Curve of \mname on \textit{de novo} Molecule Generation
%%% plot_fscore_t.py 
}
\label{fig:learning_curve}
\end{figure}
\fi 









% \subsection{Distribution of the Target Properties }
% \label{sec:distribution_of_property}

% We show the distributions of target properties (JNK3, GSK3\bm{$\beta$}, QED and LogP) of the generated molecule of \mname in Figure~\ref{fig:distribution_of_property}. 
% We also show the distribution on ZINC databases as reference. 

% \begin{figure}[h!]
% \centering
% \subfigure[JNK3 and GSK3\bm{$\beta$}]{
% \includegraphics[width=4cm]{figure/scatter_jnk_gsk.png}}
% \subfigure[QED and LogP]{
% \includegraphics[width=4cm]{figure/scatter_qed_logp.png}}
% \caption{Distributions of target properties for (a) \mname (blue) and (b) ZINC database (red). 
% We find that the generated molecules are superior to ZINC molecules on JNK3 and GSK3\bm{$\beta$}. On QED and LogP, it is also competitive compared with ZINC database. 
% %%%  plot_scatter_*.py 
% }
% \label{fig:distribution_of_property}
% \end{figure}

% \subsection{Case Study on De Novo Molecule Design}
% \label{sec:casestudy_denovo_appendix}
% We show two case studies for \textit{de novo} molecule design in Figure~\ref{fig:case_denovo_qedlogpjnkgsk}. 
% We start from scratch.  
% We found that our method is able to generate drug-like molecules with desirable properties within 10 generations . 

% \begin{figure}[h!]
% \centering
% \subfigure[]{
% \includegraphics[width=14cm]{figure/case_denovo_qedlogpjnkgsk.png}}
% \subfigure[]{
% \includegraphics[width=14cm]{figure/case_denovo_qedlogpjnkgsk2.png}}
% \subfigure[]{
% \includegraphics[width=14cm]{figure/case_study_denovo.png}}
% \caption{
% Case Study on \textit{de novo} Molecule Generation. 
% For each molecule, we show its (1) objective function as well as (2) QED, (3) LogP, (4) JNK3 and (5) GSK3\bm{$\beta$} score.
% %%%  casestudy_qedlogpjnkgsk.py 
% }
% \label{fig:case_denovo_qedlogpjnkgsk}
% \end{figure}




% \subsection{Case Study on Goal-Directed Molecule Optimization}
% \label{sec:casestudy_goal_appendix}

% In this section, we analysis some cases on goal-directed molecule optimization task in Figure~\ref{fig:case_goal_qedlogpjnkgsk}. 


% \begin{figure}[h!]
% \centering
% \subfigure[]{
% \includegraphics[width=14cm]{figure/case_denovo_qedlogpjnkgsk.png}}
% \caption{
% Case Study on Goal-Directed Molecule Optimization. 
% %%%  casestudy_qedlogpjnkgsk.py 
% }
% \label{fig:case_goal_qedlogpjnkgsk}
% \end{figure}

% \subsection{Example of Generated Molecule}

% In this section, we show some examples of generated molecules with high properties to highlight the superiority of our method in Figure~\ref{fig:example}. 



% \iffalse
% \subsection{Ablation Study} 
% \label{sec:ablation}
% Then we conduct ablation studies to explore the empirical effect of two important components of \mname. 

% As described in Section~\ref{sec:differentiable}, during molecule sampling, we sample the new molecule from the differentiable scaffolding tree (Equation~\ref{eqn:sample}). 
% We compare with a \textit{random-walk sampler}, where the topological edition (i.e., expand, shrink or unchange) and substructure are both selected randomly. 
% We consider the following variants:
% \begin{itemize}
%  \item ``\mname+DPP''. Both topology  and substructure to fill are sampled from the optimized differentiable scaffolding tree, as shown in Equation~\eqref{eqn:sample}.  
%  \item ``random + DPP''. Changing topology randomly, that is, at each leaf node, ``expand'', ``shrink'' and ``unchange'' probabilities are fixed to $0.5, 0.1, 0.4$. Substructure selection is sampled from the substructures' distribution in the optimized differentiable scaffolding tree. Then it uses DPP (Section~\ref{sec:dpp}) to select diverse and desirable molecules for the next iteration. 
%  \item ``\mname+top-$K$''. Same as ``\mname + DPP'', it uses \mname to sample new molecules. The difference is when selecting molecules for the next iteration, it selects the top-$K$ molecules with highest $f$ score. It is equivalent to $\lambda \xrightarrow[]{}+\infty$ in Equation~\eqref{eqn:dpp_obj}. 
% \end{itemize}
% We show the results in Figure~\ref{fig:ablation}. 
% \fi


% \begin{enumerate}
% \item {DST sampling v.s. random walk}. 
% \item {DPP v.s. top-$K$}. As described in Section~\ref{sec:dpp}, during each iteration, after we sampling from \mname, we utilize \textit{determinantal point process (DPP)} based selection strategy to diversify the generated molecules while maintaining the desirable properties for the next iteration. 
% In contrast, traditional genetic algorithm usually leverage \textit{top-K} strategy, that is, during all the proposed molecules, the $K$ molecules with highest objective value are selected for the next iteration. 
% Based on the formulation in Equation~\eqref{eqn:dpp_obj}, when the $\lambda$ goes to positive infinity, our DPP strategy reduces to top-$K$ strategy. 
% We compare the following variants 
% \begin{itemize}
%  \item DPP-I. Fixing $\lambda$. $\lambda=2$ performs best among $\lambda \in \{0.5, 1, 2, 5\}$. 
%  \item DPP-II. Gradually enlarge $\lambda$ linearly as generation number grows, from 1 to 3.  
%  \item DPP-III. Gradually shrink $\lambda$ linearly as generation number grows, from 3 to 1. 
%  \item ``random + random''. , then it randomly select diverse and desirable molecules for the next iteration. 
%  \item \mname topology + random substructure. Selecting substructure from the vocabulary $\calS$ randomly while topological edition is based on the differentiable scaffolding tree. 
%  \item random topology + random substructure. Both topology and substructure are selected randomly. The random sampling strategy follows random-topology and random-substructure above. 
% The results are shown in Table~\ref{table:ablation1}. 
% \end{itemize}
% We also track the change of $\log \det(V_{\cal})$ and $\log \det(S_{\cal})$ to better observe their weights in the whole objective defined in Equation~\eqref{eqn:dpp_obj}, which controls desirable properties and diversity, respectively. 
% \end{enumerate}







% \begin{table*}[h!]
% \tiny
% \centering
% \caption{Ablation study II: DPP v.s. top-$K$. 
% }
% \label{table:ablation2}
%  \resizebox{1\textwidth}{!}{
% \begin{tabular}{lccccccc}
% \toprule[0.6pt]
% Method & Novelty & Diversity & $f$ &  GSK3{$\beta$} & JNK3 & QED & LogP   \\ \hline 
% top-$K$ & & & & & & & \\ 
% DPP-I & & & & & & & \\ 
% DPP-II & & & & & & & \\ 
% DPP-III & & & & & & & \\ 
% \bottomrule[0.6pt]
% \end{tabular}}
% \end{table*}

\subsection{Additional results of \textit{de novo} molecular generation}
\label{sec:additional}

In this section, we present some additional results of \textit{de novo} molecular generation for completeness. 



First, we present the optimization curve for all the optimization tasks in Figure~\ref{fig:optimization_curve}. We observe that our method is able to reach a high objective value efficiently within 10 iterations in all the optimization tasks. 
Worth mentioning that when optimizing LogP, the model successfully learned to add a six-member ring each step, as shown in Figure~\ref{fig:logp_growing}, and the objective ($F$) value grows linearly as a function of iteration number, which is theoretically the optimal strategy under our setting. 
Then, in Figure~\ref{fig:highest_example}, we show the molecules with the highest objective ($F$) scores generated by the proposed method on optimizing QED and  ``QED+SA+JNK3+GSK3\bm{$\beta$}''. 
Then we compare our method with baseline methods on 3 molecules with the highest objective ($F$) scores in Table~\ref{table:denovo_top} and~\ref{table:denovo_multi_top} for single-objective and multi-objective generation, respectively.  


\begin{figure}[h!]
\centering
\subfigure[LogP]{
\includegraphics[width=0.32\linewidth]{figure/curve_logp.png}}
\subfigure[JNK3]{
\includegraphics[width=0.32\linewidth]{figure/curve_jnk.png}}
\subfigure[GSK3\bm{$\beta$}]{
\includegraphics[width=0.32\linewidth]{figure/curve_gsk.png}}
\subfigure[QED]{
\includegraphics[width=0.32\linewidth]{figure/curve_qed.png}}
\subfigure[JNK3+GSK3\bm{$\beta$}]{
\includegraphics[width=0.32\linewidth]{figure/curve_jnkgsk.png}}
\subfigure[QED+SA+JNK3+GSK3\bm{$\beta$}]{
\includegraphics[width=0.32\linewidth]{figure/curve_qedsajnkgsk.png}}
\caption{
The optimization curves in \textit{de novo} optimization experiments. The objective value ($F$) is a function of iterations.  }
\label{fig:optimization_curve}
\end{figure}

\begin{figure}[h!]
\centering
\includegraphics[width=\linewidth]{figure/dsf_logp.pdf}
\caption{
The first eight steps in \textit{the de novo} optimization procedure of LogP. The model successfully learned to add a six-member ring each step. }
\label{fig:logp_growing}
\end{figure}

\begin{figure}[h!]
\centering
% \subfigure[10 molecules with highest JNK3 scores]{
% \includegraphics[width=13.5cm]{figure/best_jnk.png}}
% \subfigure[10 molecules with highest GSK3\bm{$\beta$} scores]{
% \includegraphics[width=13.5cm]{figure/best_gsk.png}}
% \subfigure[10 molecules with highest average JNK3 and GSK3\bm{$\beta$} scores]{
% \includegraphics[width=13.5cm]{figure/best_jnkgsk.png}}
\subfigure[Molecules with highest average QED, normalized-SA, JNK3 and GSK3\bm{$\beta$} scores, four scores represent QED, raw SA, JNK3, and GSK3\bm{$\beta$} scores, respectively. ]{\includegraphics[width=13.5cm]{figure/best_qedsajnkgsk.png}}
\subfigure[Molecules with highest QED. ]{\includegraphics[width=13.5cm]{figure/best_qed.png}}
\caption{
Sampled molecules with the highest scores. }
\label{fig:highest_example}
\end{figure}

% QED SA JNK GSK 
% TOP-10
% Clc1ncn(-c2ccc(Nc3nccc(-c4ccccc4)n3)cc2)n1 0.60 2.25 0.93 0.83
% Fc1ccc(Nc2nccc(-c3ccccc3)n2)cc1 0.77 1.67 0.72 0.85
% c1ccc(Nc2nccc(-c3ccc(-n4cccn4)cc3)n2)cc1 0.61 1.99 0.83 0.89
% Clc1ccc(Nc2nccc(-c3ccccc3)n2)cc1 0.76 1.66 0.74 0.83
% c1ccc(Nc2nccc(-c3ccccc3)n2)cc1 0.76 1.59 0.7 0.87
% Clc1ccc(Nc2nccc(-c3ccc(Cl)cc3)n2)cc1 0.72 1.74 0.76 0.85
% Oc1ccc(-c2ccnc(Nc3ccc(Cl)cc3)n2)cc1 0.75 1.82 0.76 0.8
% O=Nc1ccc(-c2ccnc(Nc3ccccc3)n2)cc1 0.72 2.07 0.71 0.87
% c1ccc(Nc2nccc(-c3ccc(N4CCCCC4)cc3)n2)cc1 0.74 1.87 0.69 0.87
% Cc1ccc(Nc2nccc(-c3ccccc3)n2)cc1 0.76 1.64 0.71 0.82


\begin{table*}[h!]
\tiny
\centering
\caption{Highest scores of generated molecules on single-objective \textit{de novo} molecular generation. We present the result of \mname in the first 50 iterations, but please note the setting of generation varies among the models, and a completely fair comparison is impossible. }
\label{table:denovo_top}
 \resizebox{0.90\textwidth}{!}{
\begin{tabular}{lccc|ccc|ccc}
\toprule[0.6pt]
\multirow{2}{*}{Method} & \multicolumn{3}{c}{JNK3} & \multicolumn{3}{c}{GSK3\bm{$\beta$}} & \multicolumn{3}{c}{LogP} \\
& 1st & 2nd & 3rd & 1st & 2nd & 3rd  & 1st & 2nd & 3rd \\
\hline 
GCPN &  0.57 & 0.56 & 0.54  & 0.57 & 0.56 & 0.56  & 8.0 & 7.9 & 7.8 \\
MolDQN & 0.64 & 0.63 & 0.63 & 0.54 & 0.53 & 0.53  & 11.8 & 11.8 & 11.8  \\ 
GA+D & 0.81 & 0.80 & 0.80 & 0.79 & 0.79 & 0.78 & 20.5 & 20.4 & 20.2 \\
RationaleRL & 0.90 & 0.90 & 0.90  & 0.93 & 0.92 & 0.92 & - & - & - \\
MARS & 0.92 & 0.91 & 0.90 & \bf 0.95 & 0.93 & 0.92  & 45.0 & 44.3 & 43.8 \\
\mname & \bf 0.97 & \bf 0.97 &\bf 0.97 &\bf 0.95 &\bf 0.95 &\bf 0.95 &\bf 49.1 &\bf 49.1 &\bf 49.1 \\ 
\bottomrule[0.6pt]
\end{tabular}}
\end{table*}


\begin{table*}[h!]
\tiny
\centering
\caption{Highest scores of generated molecules on multi-objective \textit{de novo} molecular generation. The score is the average value of all objectives.   }
\label{table:denovo_multi_top}
 \resizebox{0.780\textwidth}{!}{
\begin{tabular}{lccc|ccc}
\toprule[0.6pt]
\multirow{2}{*}{Method} & \multicolumn{3}{c}{JNK3+GSK3\bm{$\beta$}} & \multicolumn{3}{c}{QED+SA+JNK3+GSK3\bm{$\beta$}} \\ 
& top-1 & top-2 & top-3 & top-1 & top-2 & top-3 \\
\hline 
GCPN & 0.31 & 0.31 & 0.30 & 0.57 & 0.56 & 0.56 \\ 
MolDQN & 0.46 & 0.45 & 0.45 & 0.45 & 0.45 & 0.44 \\
GA+D & 0.68 & 0.68 & 0.67 & 0.71 & 0.70 & 0.70\\
RationaleRL & 0.81 & 0.81 & 0.81  & 0.76 & 0.76 & 0.75 \\
MARS & 0.78 & 0.78 & 0.77 & 0.72 & 0.72 & 0.72 \\
\mname & \bf 0.89 & \bf 0.89 & \bf 0.89 & \bf 0.83 & \bf 0.83 & \bf 0.83 \\
\bottomrule[0.6pt]
\end{tabular}}
\end{table*}


\subsection{\textit{De novo} molecular optimization on QED (potential limitation of \DST)}
\label{sec:qed}

% On the other hand, the result of optimizing QED indicates one current limitation of \mname (see Table~\ref{table:denovo_qed} in Appendix). Unlike other tasks, \mname cannot reach the same level as other baseline methods in QED optimization. We conclude that this is due to the limitation of the expressive power of scaffolding tree itself. QED is a property that is highly dependent on \textit{how} substructures connect~\cite{bickerton2012quantifying}, while our scaffolding tree currently ignores this information. This behavior impedes the training of GNN (see learning curves in Appendix Figure~\ref{fig:loss}) and leads to the relatively poor performance. Please see Section~\ref{sec:qed} for detailed experimental setup. 

As we have touched in Section~\ref{sec:denovo}, the optimization on QED is not as satisfactory as other oracles. We compare the performance of various methods on single-objective \textit{de novo} molecular generation for optimizing QED score and show the result in Table~\ref{table:denovo_qed}. Additional baseline methods include JTVAE (junction tree variational autoencoder)~\cite{jin2018junction} and GraphAF (Graph Flow-based Autoregressive Model)~\cite{shi2019graphaf}. 
The main reason behind this result is that our GNN predicts the target property based on a scaffolding tree instead of a molecular graph, as shown in Equation~\eqref{eqn:gnn_prediction}. A scaffolding tree omits rings' assembling information, as shown in Figure~\ref{fig:adj}. 
Compared with other properties like LogP, JNK3, GSK3\bm{$\beta$}, drug-likeness is more sensitive to \textit{how} substructures connect~\cite{bickerton2012quantifying}. This behavior impedes the training of GNN and leads to the failure of optimization. 
We report the learning curve in Figure~\ref{fig:loss}, where we plot the normalized loss on the validation set as a function of epoch numbers when learning GNN. 
For fairness of comparison, validation loss is normalized by dividing the validation loss at scratch (i.e., 0-th epoch) so that all the validation losses are between 0 and 1. 
For most of the target properties, the normalized loss value on the validation set would decrease significantly, and GNN can learn these properties well, except QED. 
It verifies the failure of training the GNN on optimizing QED. 
A differentiable molecular graph at atom-wise resolution may potentially solve this problem. 
\begin{table}[h!]
\centering
\caption{Comparison of different methods on optimizing QED for single-objective \textit{de novo} molecular generation. {The results for baseline methods are copied from~\cite{You2018-xh,zhou2019optimization,shi2019graphaf,xie2021mars}. The results of JTVAE are copies from \cite{You2018-xh}}. }
\label{table:denovo_qed}
\resizebox{0.40\textwidth}{!}{
\begin{tabular}{lccc}
\toprule[0.6pt]
Method & top-1 & top-2 & top-3 \\ \hline 
JTVAE~\cite{jin2018junction} & 0.925 & 0.911 & 0.910 \\ 
GCPN~\cite{You2018-xh} & \bf 0.948 & 0.947 & 0.946 \\
MolDQN~\cite{zhou2019optimization} & \bf 0.948 & \bf 0.948 &\bf 0.948  \\
GraphAF~\cite{shi2019graphaf} & \bf 0.948 & \bf 0.948 & 0.947 \\ 
MARS~\cite{xie2021mars} & \bf 0.948  & \bf 0.948 & \bf 0.948 \\
\mname & 0.947 & 0.946 & 0.946 \\ 
\bottomrule[0.6pt]
\end{tabular}}
\end{table}

\begin{figure}[h!]
\centering
% \subfigure[LogP]{
% \includegraphics[width=0.31\linewidth]{figure/learning_curve_validloss_LogPraw.png}}
% \subfigure[GSK3B]{
% \includegraphics[width=0.31\linewidth]{figure/learning_curve_validloss_GSK3B.png}}
% \subfigure[QED]{
% \includegraphics[width=0.31\linewidth]{figure/learning_curve_validloss_QED.png}}
\includegraphics[width=0.45\linewidth]{figure/learning_curve_validloss_whole.png}
\caption{Normalized validation loss-epoch learning curves. 
For fairness of comparison, validation loss is normalized by dividing the validation loss at scratch (i.e., 0-th epoch) so that all the validation losses are between 0 and 1. 
For most of the target properties, the normalized loss value on the validation set would decrease significantly, and GNN can learn these properties well, except QED. The key reason for the failure of GNN on optimizing QED is the limitation of the expressive power of scaffolding tree itself. 
QED is a property that is highly dependent on \textit{how} substructures connect~\cite{bickerton2012quantifying}, while our scaffolding tree currently ignores that information. 
See Section~\ref{sec:qed} for more details and analysis.  
}
\label{fig:loss}
\end{figure}
% src/plot_learning_curve.py


\subsection{Results Analysis for Distribution Learning Methods (LigGPT)}
As showed in Table~\ref{table:denovo_single} and~\ref{table:denovo_multi}, distribution learning methods (LigGPT)~\cite{bagal2021liggpt} have much weaker optimization ability. 
DST and all the other baselines fall into the category of goal-directed molecule generation, a.k.a., molecule optimization, which generates molecules with high scores for a given oracle. In contrast, LigGPT belongs to distribution learning (a different category of method), which learns the distribution of the training set. We refer to \cite{brown2019guacamol} for more description of two categories of methods.
Consequently, conditioned generation learns from the training set, is unable to generate molecules with property largely beyond the training set distribution and can not optimize a property directly, even though they claim to be able to solve the same problem.  
Problem formulation of distribution learning methods leads to an inability to generate molecules with property largely beyond the training set distribution, which means they are much weaker in optimization. 


% The reason is the training dataset contains a large fraction of molecules with QED larger than 0.5 but most of them have LogP smaller than 5, JNK3 and GSK3B less than 0.1, validating the analysis above. 
% Following the original paper, the LigGPT is trained on the 100K labeled molecules, with default hyperparameters. We target 10 (beyond the maximum of the dataset) for LogP and 1 (upper bound) for other oracles. results are 




\subsection{Ablation study}
\label{sec:ablation}
As described in Section~\ref{sec:differentiable}, during molecule sampling, we sample the new molecule from the differentiable scaffolding tree (Equation~\ref{eqn:sample}). To verify the effectiveness of our strategy, we compare with a \textit{random-walk sampler}, where the topological edition (i.e., expand, shrink or unchange) and substructure are both selected randomly. 
% Worth mentioning that to we evaluate \mname and other variants in a challenging setting, i.e., for all the methods, each iteration, only 3 molecules are selected for the next iteration, i.e., $C=3$, unlike $C=10$ above. 
We consider the following variants:
\begin{itemize}
 \item ``\mname + DPP''. Both topology and substructure to fill are sampled from the optimized differentiable scaffolding tree, as shown in Equation~\eqref{eqn:sample}. 
 This is what we use in this paper. 
 \item ``random + DPP''. Changing topology randomly, that is, at each leaf node, ``expand'', ``shrink'' and ``unchange'' probabilities are fixed to $0.5, 0.1, 0.4$. Substructure selection is sampled from the substructures' distribution in the optimized differentiable scaffolding tree. Then it uses DPP (Section~\ref{sec:dpp}) to select diverse and desirable molecules for the next iteration. 
 \item ``\mname + top-$K$''. Same as ``\mname + DPP'', it uses \mname to sample new molecules. The difference is when selecting molecules for the next iteration, it selects the top-$K$ molecules with highest $f$ score. It is equivalent to $\lambda \xrightarrow[]{}+\infty$ in Equation~\eqref{eqn:dpp_obj}. 
\end{itemize}
We show the results in Figure~\ref{fig:ablation}. We find that both \mname sampling and DPP-based diversification play a critical role in performance. 
We check the results for ``\mname + top-K'', during some period, the objective does not grow, we find it is trapped into local minimum, impeding its performance, especially convergence efficiency. 
``random+DPP'' exhibits the random-walk behaviour and it would not reach satisfactory performance. 
When optimizing LogP, ``\mname+DPP'' and ``\mname+top-$K$'' achieved similar performance, because logP score will prefer larger molecules with more carbon atoms, which is less sensitive to the diversity and relatively easier to optimize. Overall, ``\mname+DPP'' is the best strategy compared with other variants. 

\begin{figure}[h!]
\centering
\subfigure[JNK3]{
\includegraphics[width=0.32\linewidth]{figure/ablation_jnk.png}}
\subfigure[GSK3B]{
\includegraphics[width=0.32\linewidth]{figure/ablation_gsk.png}}
\subfigure[LogP]{
\includegraphics[width=0.32\linewidth]{figure/ablation_logp.png}}
\caption{Ablation study. Objective value ($F$) as a function of iterations. See Section~\ref{sec:ablation} for more details. 
}
\label{fig:ablation}
\end{figure}


\subsection{Chemical space visualization}
\label{sec:visualize_chemical}

We use principle component analysis (PCA) to visualize the distribution of explored chemical structures in optimizing ``JNK3 \& GSK3\bm{$\beta$}''. 
Specifically, we fit a two-dimensional principal component analysis (PCA)~\cite{bro2014principal} for 2048-bit Morgan fingerprint vectors of 20K ZINC molecules, which are randomly selected from ZINC database~\cite{sterling2015zinc}. 
Then we use the PCA to project the fingerprint of the generated molecule from various generations into a two-dimensional vector to observe their trajectories. The results are reported in Figure~\ref{fig:pca}, 
where the grey points represent the two-dimensional vector of ZINC molecules. 
We find that our method explores different parts of the 2D projection of the chemical space and covers a similar chemical space as the ZINC database after 20 to 30 iterations. 
% It finding different parts of the chemical space and exhibit high diversity. 
% In addition, it converges rapidly within 30 generations, validating the efficiency of \mname.


\begin{figure}[h!]
\centering
\subfigure[After 3 iterations]{
\includegraphics[width=0.32\linewidth]{figure/pca_3.png}}
\subfigure[After 5 iterations]{
\includegraphics[width=0.32\linewidth]{figure/pca_5.png}}
\subfigure[After 10 iterations]{
\includegraphics[width=0.32\linewidth]{figure/pca_10.png}}
\subfigure[After 20 iterations]{
\includegraphics[width=0.32\linewidth]{figure/pca_20.png}}
\subfigure[After 30 iterations]{
\includegraphics[width=0.32\linewidth]{figure/pca_30.png}}
\caption{
Visualization of chemical space covered during optimization. We used PCA to reduce the dimension of Morgan fingerprint. The gray points are the ZINC 250k data set. while colored points are generated molecules after corresponding iterations.}
\label{fig:pca}
\end{figure}

\subsection{Additional Interpretability Analysis}
\label{sec:appendix_interpretability}


\begin{figure}[h!]
\centering
\includegraphics[width=0.6\linewidth]{figure/interpret_logp.png}
\caption{Interpretability analysis when optimizing LogP. }
\label{fig:interpret_logp}
\end{figure}

We provide an interpretability example in Figure~\ref{fig:interpret_logp}. At the leaf node (yellow), from the optimized differentiable scaffolding tree, we find that the leaf weight and expand weight are both 0.99. Thus we decide to EXPAND, the six-member ring is selected and filled in the expansion node (blue). This is consistent with our intuition that logP score will prefer larger molecules with more carbon atoms. 
% The node weights and local gradient values provide interpretability at the substructure level. A positive gradient on expanding node means a positive contribution to the objective value increment, while a negative gradient on a leaf node means a negative contribution.





==> DST arxiv/experiment.tex <==






\section{Experiment}
\label{sec:experiment}

% In this section, we first describe the experimental setup in section~\ref{sec:setup} following~\cite{jin2018junction,jin2019learning,You2018-xh,shi2019graphaf,jin2020multi,xie2021mars}. Then we analyze the result from three aspects: optimization performance, oracle efficiency, and interpretability.

\subsection{Experimental Setup}
\label{sec:setup}
% In this section, we briefly describe the basic experimental setup, mainly following~\cite{jin2018junction,jin2019learning,You2018-xh,shi2019graphaf,jin2020multi,xie2021mars}. More implementation details are provided in Appendix. 
% \noindent\textbf{Task}. We focus on the following two optimization tasks:
% (1) \textbf{molecular modification} 
% % (Section~\ref{sec:goal_directed}) 
% % and
% (2) \textbf{de novo molecule generation}.  
% % (Section~\ref{sec:denovo}). 



% \marked{Following~\cite{jin2020multi,xie2021mars} the target molecular properties}, 
\noindent\textbf{Molecular Properties} contains \textbf{QED}; 
\textbf{LogP}; 
\textbf{SA}; 
\textbf{JNK3}; 
\textbf{GSK3\bm{$\beta$}}, \marked{following~\cite{jin2020multi,nigam2019augmenting,moss2020boss,xie2021mars}, where QED quantifies drug-likeness; LogP indicates the water-octanol partition coefficient; SA stands for synthetic accessibility and is used to prevents the formation of chemically unfeasible molecules; JNK3/GSK3$\bm{\beta}$ measure inhibition against c-Jun N-terminal kinase-3/Glycogen synthase kinase 3 beta. }
% QED, JNK3 and GSK3\bm{$\beta$} scores range from 0 to 1. 
% LogP score range from $-\infty$ to $+\infty$ while SA score ranges from 1 to 10. 
% We normalize SA to $[0,1]$ for multi-objective generation. 
For all the 5 scores (including normalized SA), higher is better. 
We conducted (1) single-objective generation that optimizes JNK3, GSK3\bm{$\beta$} and LogP separately
and (2) multi-objective generation that optimizes the mean value of  ``JNK3+GSK3\bm{$\beta$}'' and ``QED+SA+JNK3+GSK3\bm{$\beta$}'' in the main text. 
Details are in Section~\ref{sec:property}. 




\noindent\textbf{Dataset}: ZINC 250K contains around 250K druglike molecules~\cite{sterling2015zinc}. 
% To select the substruture set $\calS$, we break the molecules into substructures (including single rings and single atoms), 
We select the substructures that appear more than 1000 times in ZINC 250K as the vocabulary set $\calS$, which contains 82 most frequent substructures. Details are in Section~\ref{sec:dataset}. 
% \js{can we provide some justification of the choice of 1K times requirement. Are 82 substructures sufficient to generate most molecules? }




\noindent\textbf{Baselines}. 
(1) \textbf{LigGPT} (string-based distribution learning model with Transformer as a decoder)~\cite{bagal2021liggpt}; 
(2) \textbf{GCPN} (Graph Convolutional Policy Network)~\cite{You2018-xh}; 
(3) \textbf{MolDQN} (Molecule Deep Q-Network)~\cite{zhou2019optimization}; 
(4) \textbf{GA+D} (Genetic Algorithm with Discriminator network)~\cite{nigam2019augmenting};  
(5) \textbf{MARS} (Markov Molecular Sampling)~\cite{xie2021mars}; 
(6) \textbf{RationaleRL}~\cite{jin2020multi}; 
\marked{
(7) \textbf{ChemBO} (Chemical Bayesian Optimization)~\cite{korovina2020chembo}; 
(8) \textbf{BOSS} (Bayesian Optimization over String Space)~\cite{moss2020boss}. } 
Among them, LigGPT belongs to deep generative model, where all the oracle calls can be precomputed; 
GCPN, MolDQN are deep reinforcement learning methods; 
GA+D, MARS are evolutionary learning methods; 
RationaleRL is deep generative model fine-tuned with RL techniques. 
\marked{ChemBO and BOSS are Bayesian optimization methods. We also consider a \mname variant: \textbf{\mname-rand}. Instead of optimizing and sample from \mname, \mname-rand leverages random local search, i.e., randomly selecting basic operations (EXPAND, REPLACE, SHRINK) and substructure from vocabulary. To improve efficiency, we also select a subset of all the random samples with high surrogate GNN prediction scores. } 
All the baselines except LigGPT require online oracle calls.
Details are in Section~\ref{sec:baseline}. 
% Detailed setup for baseline methods are described in Section~\ref{sec:baseline} in Appendix. 


\noindent\textbf{Metrics}. 
\marked{For each method, we select top-100 molecules with highest property scores for evaluation, and consider the following metrics following~\cite{jin2018junction,You2018-xh,jin2020multi,xie2021mars}}
(1) \textbf{Novelty (Nov)} \marked{(\% of the generated molecules that are not in training set)}; 
(2) \textbf{Diversity (Div)} \marked{(average pairwise Tanimoto distance between the Morgan fingerprints)}; 
(3) \marked{\textbf{Average Property Score (APS)} (average score of top-100 molecules)};
% \marked{\footnote{\marked{For single-objective design, the success criteria are JNK3/GSK3\bm{$\beta$}$\geq 0.5$ and LogP$\geq5.0$ respectively. For multi-objective design, the criteria is average of all the normalized target property scores is greater than 0.4. }}};
(4) \textbf{\# of oracle calls}: \mname needs to call oracle in labeling data for GNN (\textbf{precomputed}) and \mname based \textit{de novo} generation (\textbf{online}), we show the costs for both steps. \marked{For each method in Table~\ref{table:denovo_multi} and~\ref{table:denovo_single}, we set the number of oracle calls so that the property score nearly converge w.r.t. oracle call’s number. }
% Since we only enumerate valid chemical structures during the recovery from scaffolding trees (Section~\ref{sec:assemble}), the chemical validities are always 100\%. 
Details are in Section~\ref{sec:metrics}. 




\begin{table*}[h!]
\tiny
% \centering
% \caption{Multi-objective \textit{de novo} molecular generation. }
%  \resizebox{0.70\textwidth}{!}{
\parbox{.25\textwidth}{\caption{Multi-objective \textit{de novo} design. \#oracle = (1)``\textbf{precomputed} oracle call'' (to label molecules in existing database) + (2)``\textbf{online} oracle call'' (during learning). }
\label{table:denovo_multi}
}
\hspace{0.03\textwidth}
\parbox{.60\textwidth}{
\centering
\begin{tabular}{lcccc|cccc}
\toprule[0.6pt]
\multirow{2}{*}{Method} & \multicolumn{4}{c}{JNK3+GSK3\bm{$\beta$}} & \multicolumn{4}{c}{QED+SA+JNK3+GSK3\bm{$\beta$}} \\ 
& Nov$\uparrow$ & Div$\uparrow$ & {APS}$\uparrow$ & \#oracle$\downarrow$ & Nov$\uparrow$ & Div$\uparrow$ & {APS}$\uparrow$ & \#oracle$\downarrow$ \\
\hline 
LigGPT & \textbf{100\%} & \textbf{0.845} & 0.271 & 100k+0 & \textbf{100\%} & \textbf{0.902} & 0.378 & 100k+0 \\ 
GCPN & \textbf{100\%} & 0.578 & 0.293 & 0+200K & \textbf{100\%} & 0.596 & 0.450 & 0+200K \\ 
MolDQN & \textbf{100\%} & 0.605 & 0.348 & 0+200K & \textbf{100\%} & 0.597 & 0.365 & 0+200K \\ 
GA+D & \textbf{100\%} & 0.657 & 0.608 & 0+50K & 97\% & 0.681 & 0.632 & 0+50K \\ 
RationaleRL & \textbf{100\%} & 0.700 & 0.795 & 25K+67K & 99\% & 0.720 & 0.675 & 25K+67K \\ 
MARS & \textbf{100\%} & 0.711 & 0.789 & 0+50K  & \textbf{100\%} & 0.714 & 0.662 & 0+50K \\ 
{ChemBO} & 98\% & 0.702 & 0.747 & 0+50K & 99\% & 0.701 & 0.648 & 0+50K \\ 
{BOSS} & 99\% & 0.564 & 0.504 & 0+50K & 98\% & 0.561 & 0.504 & 0+50K \\ 
{\mname-rand} & \textbf{100\%} & 0.456 & 0.622 & 10+5K & \textbf{100\%} & 0.765 & 0.575 & 20K+5K \\ 
\mname & \textbf{100\%} &  0.750 & \textbf{0.827} & \textbf{10K+5K} & \textbf{100}\% &  0.755 & \textbf{0.752} & \textbf{20K+5K} \\ 
\bottomrule[0.6pt]
\end{tabular}}
\end{table*}










% \begin{table*}[h!]
% \tiny
% \centering
% \caption{Multi-objective \textit{de novo} molecular generation. }
% \label{table:denovo_multi}
%  \resizebox{0.70\textwidth}{!}{
% \begin{tabular}{lcccc|cccc}
% \toprule[0.6pt]
% \multirow{2}{*}{Method} & \multicolumn{4}{c}{JNK3+GSK3\bm{$\beta$}} & \multicolumn{4}{c}{QED+SA+JNK3+GSK3\bm{$\beta$}} \\ 
% & Nov$\uparrow$ & Div$\uparrow$ & SR$\uparrow$ & \#oracle$\downarrow$ & Nov$\uparrow$ & Div$\uparrow$ & SR$\uparrow$ & \#oracle$\downarrow$ \\
% \hline 
% LigGPT & \textbf{100\% & \textbf{0.843 & 0.0\% & 100k+0 & 100\% & \textbf{0.906 & 2.84\% & 100k+0   \\ 
% GCPN & \textbf{100\% & 0.583 & 0.0\% & 0+200K & \textbf{100\% & 0.590 & 12.7\% & 0+200K \\ 
% MolDQN & \textbf{100\% & 0.605 & 2.8\% & 0+200K & \textbf{100\% & 0.599 & 1.0\% & 0+200K\\ 
% GA+D & 97.4\% & 0.660 & 48.0\% & 0+50K & 96.4\% & 0.688 & 35.4\% & 0+50K \\ 
% RationaleRL & 93.6\% & 0.700 & 82.8\% & 25K+67K & 94.0\% & 0.720 & 75.3\% & 25K+67K \\ 
% MARS & 97.9\% & 0.699 & 80.2\% & 0+50K  & 98.4\% & 0.714 & 73.4\% & 0+50K \\ 
% \mname & 97.5\% &  0.745 & \textbf{92.0\% & \textbf{10K+5K & 98.8\% &  0.774 & \textbf{79.8\% & \textbf{20K+5K \\ 
% \bottomrule[0.6pt]
% \end{tabular}}
% \end{table*}


\subsection{Optimization Performance}
\label{sec:denovo}
% \js{The performance of GCPN and MolDQN are very poor in SR. Do we have an explanation? We should make sure to avoid reviewers question the validity of our experiments.} \tf{in both RationaleRL and MARS paper, GCPN is the worst baseline. }
% The de novo generation is to design novel, diverse molecule with desirable chemical properties from scratch. 
% We consider (1) single-objective generation that optimizes JNK3, GSK3\bm{$\beta$} and LogP separately
% and (2) multi-objective generation that optimize the mean value of  ``JNK3+GSK3\bm{$\beta$}'' and ``QED+SA+JNK3+GSK3\bm{$\beta$}''. 



The results of multi-objective and single-objective generation are shown in Table~\ref{table:denovo_multi} and~\ref{table:denovo_single}. 
We find that DGM (LigGPT) and RL based methods (GCPN and MolDQN) fails in some tasks, which is consistent with the results reported in RationaleRL~\cite{jin2020multi} and MARS~\cite{xie2021mars}. 
Overall, \mname obtains the best results in most tasks. 
In terms of success rate and diversity, \mname outperformed all baselines in most tasks. 
It also reached the highest scores within $T=50$ iterations in most optimization tasks (see Table \ref{table:denovo_top} and \ref{table:denovo_multi_top} in Appendix). 
Especially in optimizing LogP, the model successfully learned to add a six-member ring (see Figure~\ref{fig:logp_growing} in Appendix) each step, which is theoretically the optimal strategy under our setting. 
Combined with the ablation study comparing with random selection (see Figure \ref{fig:ablation} in Appendix), our results show the local gradient defined by \mname is a useful direction indicator, consistent with the concept of gradient. 
Further, achieving high diversity validates the effect of the DPP-based selection strategy. 
Although the novelty is not the highest, it is still comparable to baseline methods. These results show our gradient-based optimization strategy has a strong optimization ability to provide a diverse set of molecules with high objective functions. 



\begin{table*}[h!]
\tiny
\centering
\caption{Single-objective \textit{de novo} molecular generation.  }
\label{table:denovo_single}
 \resizebox{1.0\textwidth}{!}{
\begin{tabular}{lcccc|cccc|cccc}
\toprule[0.6pt]
\multirow{2}{*}{Method} & \multicolumn{4}{c}{JNK3} & \multicolumn{4}{c}{GSK3\bm{$\beta$}} & \multicolumn{4}{c}{LogP} \\ 
& Nov$\uparrow$ & Div$\uparrow$ & {APS}$\uparrow$ & \#oracle$\downarrow$ & Nov$\uparrow$  & Div$\uparrow$ & {APS}$\uparrow$ & \#oracle$\downarrow$ & Nov$\uparrow$ & Div$\uparrow$ & {APS}$\uparrow$ & \#oracle$\downarrow$ \\
\hline 
LigGPT & \textbf{100\%} & \textbf{0.837} & 0.302 & 100K+0 & \textbf{100\%} & \textbf{0.867} & 0.283 & 100K+0 & \textbf{100\%} & \textbf{0.868} & 4.56 & 100K+0 \\ 
GCPN & \textbf{100\%} & 0.584 & 0.365 & 0+200K  & \textbf{100\%} & 0.519 & 0.400 & 0+200K  & \textbf{100\%} & 0.532 & 5.43 & 0+200K \\
MolDQN & \textbf{100\%} & 0.605 & 0.459  & 0+200K & \textbf{100\%} & 0.545 & 0.398 & 0+200K  & \textbf{100\%} & 0.485 & 6.00 & 0+200K  \\
GA+D & 99\% & 0.702 & 0.615  & 0+50K & 98\% & 0.687 & 0.678 & 0+50K & \textbf{100\%} & 0.721 & 30.2 & 0+50K \\
RationaleRL & 99\% & 0.681 & 0.803 & 25K+32K & 99\% & 0.731 & 0.806 & 30K+45K & - & - & -  & - \\
MARS & \textbf{100\%} & 0.711 & 0.784  & 0+50K & \textbf{100\%} & 0.735 & 0.810 & 0+50K & \textbf{100\%} & 0.692 & 44.1 & 0+30K \\ 
{ChemBO} & 98\% & 0.645 & 0.648 & 0+50K & 98\% & 0.679 & 0.492 & 0+50K & 98\% & 0.732 & 10.2 & 0+50K \\ 
{BOSS} & 98\% & 0.601 & 0.471 & 0+50K & 99\% & 0.658 & 0.432 & 0+50K & 100\% & 0.735 & 9.64 & 0+50K  \\ 
{\mname-rand} & \textbf{100\%} & 0.754 & 0.413 & 10K+10K & 97\% & 0.793 & 0.455 & 10K+10K & \textbf{100\%} & 0.713 & 36.1 & 10K+15K \\ 
\mname & \textbf{100\%} & 0.732 & \textbf{0.928}  & \textbf{10K+5K} & \textbf{100\%} & 0.748 & \textbf{0.869}  & \textbf{10K+5K} & \textbf{100\%} & 0.704 & \textbf{47.1} & \textbf{10K+5K} \\  
\bottomrule[0.6pt]
\end{tabular}}
\end{table*}



% We have the several findings:
% \begin{itemize}[leftmargin=*]
% \item \textbf{Novelty}: almost all the methods achieve high novelty ($>$95\%), indicating that they are able to find novel drugs. 
% \item \textbf{Diversity}: our method achieves highest diversity in almost all the tasks, validating the effectiveness of DPP based selection strategy. 
% \item \textbf{success rate (SR)}: \mname demonstrates the best performance among all the compared methods in almost all the tasks, obtaining up to 10.7\% absolute improvement. Compared with single-objective generation, the improvement over baseline methods is more significant in multi-objective generation. 
% \item \textbf{number of oracle calls}: \mname costs less oracle calls compared with baseline methods thanks to its efficient exploration to the chemical space. Note that \mname costs oracle calls in two phases: (i) learning GNN phase (Section~\ref{sec:gnn}): oracle is called to acquire the groundtruth $y$; and (ii) inference phase: scoring generated molecules (Eq.~\ref{eqn:v}). 
% Compared with evolutionary learning algorithms, deep generative models such as RationaleRL usually require lots of oracle calls in selecting reference data~\cite{jin2019learning,jin2020multi}. 
% RL methods, though do not need reference data, usually requires more oracle calls due to the large variance during the learning process. 
% \end{itemize}

% We present a case study in Fig.~\ref{fig:case}(b) to illustrate how \mname grows a molecule from scratch step-by-step. 
% We find \mname can generate molecules with desirable properties from scratch within several iterations. In the beginning (the first 5 iterations), it grows the molecular scaffold by adding new substructures (i.e., EXPAND operation). During the period, the molecule size and target property scores significantly increase. Then, in the later iterations, the rough scaffolding is fixed, ``REPLACE'' is used to search the better molecules within the scaffold. In this period, the properties of the generated molecules improve slightly compared with the initial iterations, sometimes even fluctuate. 



\subsection{Oracle Efficiency}
\label{sec:oracle_experiment}
As mentioned above, oracle calls for realistic optimization tasks can be time-consuming and expensive. 
From Table~\ref{table:denovo_multi} and~\ref{table:denovo_single}, we can see that majority of de novo optimization methods require oracle calls online (instead of precomputation), including all of RL/evolutionary algorithm based baselines. \mname takes fewer oracle calls compared with baselines. \mname can leverage the precomputed oracle calls to label the molecules in an existing database (i.e., ZINC) for training the oracle GNN and dramatically saving the oracle calls during reference. 
In the three tasks in Table~\ref{table:denovo_single}, two-thirds of the oracle calls (10K) can be precomputed or collected from other sources. 
To further verify the oracle efficiency, we explore a special setting of molecule optimization where the budget of oracle calls is limited to a fixed number (2K, 5K, 10K, 20K, 50K) and compare the optimization performance.
For GCPN, MolDQN, GA+D and MARS, the learning iteration number depends on the budget of oracle calls. 
RationaleRL~\cite{jin2020multi} is not included because it requires intensive oracle calls to collect enough reference data, exceeding the oracle budget in this scenario. 
In \mname, we use around 80\% budget to label the dataset (i.e., training GNN) while the remaining budget to conduct \textit{de novo} design. Specifically, for 2K, 5K, 10K, 20K, 50K, we use 1.5K, 4K, 8K, 16K and 40K oracle calls to label the data for learning GNN, respectively. 
%  \js{How exactly can we fix the number of oracle calls for all the methods? Let's elaborate the process with fixed budget. Does lower budget mean fewer training epochs? We should comment the relationship between training epoch and oracle budget. Or this is for the inference time, how exactly can you constrain the number of oracle calls?}
% \tf{there is no inference for gcpn, moldqn, MARS and GA. we save molecules generated from learning process and evaluate them. }
We show the average objective values of top-100 molecules under different oracle budgets in Figure~\ref{fig:oracle_num}. 
Our method shows a significant advantage compared to all the baseline methods in all limited budget settings. 
We conclude the reason as supervised learning is a well-studied and much easier task than generative modeling. 
% It is also worth mentioning that our method can even perform oracle-free optimization, as we can use the trained GNN as a static surrogate, though sacrificing some optimization ability. \js{what is our performance for oracle free setting? Show it} In real cases, labeled data are usually collected for expensive oracles. We can train the GNN with those data and optimize the molecules without explicitly calling the oracle. 
\begin{figure}[h!]
\centering
% \subfigure[JNK3]{
% \includegraphics[width=4.0cm]{figure/oracle_jnk.png}}
% \subfigure[GSK3\bm{$\beta$}]{
% \includegraphics[width=4.0cm]{figure/oracle_gsk.png}}
% \subfigure[JNK3 + GSK3\bm{$\beta$}]{
% \includegraphics[width=4.0cm]{figure/oracle_jnkgsk.png}}
% \subfigure[GSK3\bm{$\beta$} todo]{
% \includegraphics[width=4cm]{figure/oracle_jnk.png}}
{\includegraphics[width=0.86\linewidth]{figure/top100_oracle_call.png}}
\caption{\marked{
Oracle efficiency test. Top-100 average score v.s. number of oracle calls. }
}
\label{fig:oracle_num}
\end{figure}

\subsection{Interpretability Analysis}
\label{sec:interpret}


\begin{figure}[h!]
\centering
\subfigure{
\includegraphics[width=0.6\linewidth]{figure/interpret_qedsajnkgsk2.png}}
\subfigure{
\includegraphics[width=0.3\linewidth]{figure/interpret_text.png}}
% {\includegraphics[width=0.6\linewidth]{figure/interpret_qedsajnkgsk2.png}}
\caption{Two steps in optimizing ``QED+SA+JNK3+GSK3\bm{$\beta$}''.  
% Positive weight gradient on expand node means a positive contribution, while negative gradient represents negative one. Due to space limit, we only show the gradient of two expand nodes. 
}
\label{fig:interpret}
\end{figure}


% \begin{figure}[h!]
% \centering
% \includegraphics[width=0.65\linewidth]{figure/interpret_qedsajnkgsk2.png}
% \caption{Two modification steps in optimizing ``QED+SA+JNK3+GSK3\bm{$\beta$}''.  Positive weight gradient on expand node means a positive contribution, while negative gradient represents negative one. Due to space limit, we only show the gradient of two expand nodes. }
% \label{fig:interpret}
% \end{figure}







To obtain more insights from the local gradient, We visualize two modification steps in Figure~\ref{fig:interpret}. 
The node weights and their gradient values interpret the property at the substructure level. 
% A positive gradient on expanding node means a positive contribution to the objective value increment, while a negative gradient represents negative one (at least locally). 
This is similar to most attribution-based interpretable ML methods, e.g., saliency map~\cite{simonyan2013deep}. 


% \subsection{Landscape of Objective Function}

% We empirically explore the landscape of objective function $F$ when growing the molecule from stratch. Specifically, we visualize the objective as a function of number of added substructures. 

% \begin{figure}
% \centering
% \includegraphics[width=6cm]{figure/landscape.png}
% \caption{Landscape of objective function $F$. }
% \label{fig:landscape}
% \end{figure}




